Encryption with Quantum Public Keys

It is an important question to find constructions of quantum cryptographic protocols which rely on weaker computational assumptions than classical protocols. Recently, it has been shown that oblivious transfer and multi-party computation can be constructed from one-way functions, whereas this is impossible in the classical setting in a black-box way. In this work, we study the question of building quantum public-key encryption schemes from one-way functions and even weaker assumptions. Firstly, we revisit the definition of IND-CPA security to this setting. Then, we propose three schemes for quantum public-key encryption from one-way functions, pseudorandom function-like states with proof of deletion and pseudorandom function-like states, respectively.

==> macros.tex <==
\RequirePackage{etex}
\ifnum\toc=1 
    \usepackage[nottoc]{tocbibind} %This adds the bibliography to the table of contents (of course, only if it exists). There is no need to add the table of contents page to the table of contents, hence the option "nottoc".
\fi
\ifnum\sigconf=0\usepackage{authblk}\fi \usepackage{silence} %authbulk must loaded before the silence package!!
\usepackage[modulo]{lineno}
\usepackage{amsthm,amssymb,amsfonts,latexsym,color,paralist,url,ifdraft,mathrsfs,thm-restate,comment,bbold,booktabs,wrapfig}


\usepackage[utf8]{inputenc} \usepackage[autostyle=false, style=english]{csquotes} \MakeOuterQuote{"}

%csquotes after inputenc
\usepackage[T1]{fontenc}
\ifnum\sigconf=0
    \ifnum \shownomenclature=1
        \usepackage[refpage,prefix]{nomencl}
        \newcommand*{\nom}[3]{#2\nomenclature[#1]{#2}{#3}} 
        \makenomenclature
        % the following part makes the nomenclature to be a section rather than a section*. It also gives it a label. In the beginning, I had a solution which was based on the following url, but it stopped working, and that's why it is commented out: https://tex.stackexchange.com/questions/124608/how-to-format-the-name-of-a-nomenclature
        %\xpatchcmd{\thenomenclature}{
        %\section*{\nomname}}{% Replace it by the following
        %\section{\nomname}\label{sec:nomenclature}
        %}{\typeout{Success!}}{\typeout{Failure}}
        
        %since the previous solution didn't work, we simply redefine the command itself. See here for the original command: https://github.com/borisveytsman/nomencl/blob/master/nomencl.dtx
  \makeatletter
        \def\thenomenclature{%
  \providecommand*{\listofnlsname}{\nomname}%
  
    
      \section{\nomname}
      \label{sec:nomenclature}    
      \if@intoc\addcontentsline{toc}{section}{\nomname}\fi%
    
  
  \nompreamble
  \if@nomentbl
    \let\itemOrig=\item
    \def\item{\gdef\item{\\}}%
    \expandafter\longtable\expandafter{\@nomtableformat}
  \else
    \list{}{%
      \labelwidth\nom@tempdim
      \leftmargin\labelwidth
      \advance\leftmargin\labelsep
      \itemsep\nomitemsep
      \let\makelabel\nomlabel}%
  \fi
}
\makeatother 
    \fi
    
    \usepackage[draft=false,pageanchor]{hyperref}
    \def\pagedeclaration#1{, \hyperlink{page.#1}{page\nobreakspace#1}} %This is needed for the nomenclature
    \usepackage{doi}

    \usepackage[final]{graphicx}
\fi

 %\usepackage{mathtools} \mathtoolsset{showonlyrefs} %the mathtools way does not work nicely with sigconf. I *think* aotunum works in all cases.
\ifdraft{\usepackage{showlabels}}{} %must be after use package{hyperref}.

%\usepackage[refpage,prefix]{nomencl} \newcommand*{\nom}[2]{#1\nomenclature{#1}{#2}} \makenomenclature
%\usepackage[displaymath,textmath,sections,graphics,floats]{preview}
%\RequirePackage{silence}
\WarningFilter{l3regex}{This package is obsolete }

\usepackage [ lambda,advantage , operators , sets , adversary , landau , probability , notions , logic ,ff, mm,primitives , events , complexity , asymptotics , keys]{cryptocode}
%the following commands are defined by crptocode. Define these ourselves if needed: \newcommand{\poly}{\mathrm{poly}} \newcommand{\prob}[1]{\Pr[ #1 ]} \newcommand{\norm}[1]{\left\| #1 \right\|} \newcommand{\RR}{\mathbb{R}} \newcommand{\FF}{\mathbb{F}} \newcommand{\CC}{\mathbb{C}} \newcommand{\NN}{\mathbb{N}}\DeclarePairedDelimiter\ceil{\lceil}{\rceil} \DeclarePairedDelimiter\floor{\lfloor}{\rfloor}
\renewcommand{\verify}{\ensuremath{\mathsf{verify}}} 


%\renewcommand{\sfdefault}{phv}
%\renewcommand{\rmdefault}{ptm}

\ifdraft{\newcommand{\authnote}[3]{{\color{#3} {\bf  #1:} #2}}}{\newcommand{\authnote}[3]{}}
\newcommand{\note}[1]{{\color{red}#1}}
%Example for how this should be used, in main file:
%\newcommand{\onote}[1]{\authnote{Or}{#1}{blue}}


\newcommand{\CNOT}{\mathrm{CNOT}}
\newcommand{\defeq}{\stackrel{\mathrm{def}}{=}}

\newcommand{\const}{\mathrm{const}}

\newcommand{\bra}[1]{\langle #1 \vert}
\newcommand{\ket}[1]{\vert #1 \rangle}
\newcommand{\ketbra}[1]{\vert #1 \rangle \langle #1 \vert}
\newcommand{\braket}[2]{\langle #1 \vert #2 \rangle}
\newcommand{\conjugate}[1]{#1^{\dagger}}
\newcommand{\tensor}{\otimes}
\DeclareMathOperator{\tr}{Tr}
\DeclareMathOperator{\Tr}{Tr}
\newcommand{\transpose}[1]{#1^{\mathsf{T}}}
\ifdraft{\linenumbers}{}

\DeclareMathOperator{\spn}{span}
\DeclareMathOperator{\E}{\mathbb{E}}

%\PreviewMacro*\onote
%\PreviewMacro*\nom
%\PreviewMacro*\ifdraft
%\DeclareMathOperator*{\E}{\scalerel*{\mathbb{E}}{\textstyle\sum}}


\newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}

%document specific
\usepackage{algorithm,algorithmicx,algpseudocode}
\usepackage[normalem]{ulem}

\newcommand{\BQP}{\textsf{BQP}}

\newcommand{\decrypt}{\ensuremath{\mathsf{decrypt}}}
\newcommand{\encrypt}{\ensuremath{\mathsf{encrypt}}}
\newcommand{\keygen}{\ensuremath{\mathsf{key\text{-}gen}}}
\newcommand{\otr}{\ensuremath{\mathsf{OTR}}}
\newcommand{\stamp}{
 {\mathchoice
  {\includegraphics[height=1.8ex]{RubberStamp}}
  {\includegraphics[height=1.8ex]{RubberStamp}}
  {\includegraphics[height=1.2ex]{RubberStamp}}
  {\includegraphics[height=0.9ex]{RubberStamp}}
 }
}
%\newcommand{\keygen}{\ensuremath{\mathsf{key\textit{-}gen}}}
\newcommand{\tokengen}{\ensuremath{\mathsf{token\textit{-}gen}}}
%\newcommand{\sign}{\ensuremath{\mathsf{sign}}}
%\newcommand{\verify}{\ensuremath{\mathsf{verify}}}


\usepackage{tikz}
\usetikzlibrary{arrows,chains,matrix,positioning,scopes}
%
\makeatletter
\tikzset{join/.code=\tikzset{after node path={%
\ifx\tikzchainprevious\pgfutil@empty\else(\tikzchainprevious)%
edge[every join]#1(\tikzchaincurrent)\fi}}}
\makeatother
%
\tikzset{>=stealth',every on chain/.append style={join},
         every join/.style={->}}
\tikzstyle{labeled}=[execute at begin node=$\scriptstyle,
   execute at end node=$]
%
\ifnum\sigconf=0
    \usepackage[capitalise]{cleveref} %Incompatible with showonlyrefs
    \crefname{Game}{Game}{Games}
\fi
\usepackage{autonum}%must be loaded after cleveref. Sometimes causes bugs. The alternative is incomaptible with cleveref:
 %\usepackage{mathtools} \mathtoolsset{showonlyrefs} %the mathtools way does not work nicely with sigconf. I *think* aotunum works in all cases. In any case, showonlyrefs does not work with cleveref.
\ifnum\sigconf=0
    \newtheorem{theorem}{Theorem} 
    \newtheorem{lemma}{Lemma}
    \newtheorem{corollary}{Corollary}
    \newtheorem{proposition}{Proposition}
    \newtheorem{definition}{Definition}
    \newtheorem{example}{Example}
    \newtheorem{conjecture}{Conjecture}
\fi 
  \newtheorem{claim}{Claim}
  \newtheorem{fact}{Fact}
  \newtheorem*{theorem*}{Theorem}
  \newtheorem*{lemma*}{Lemma}
  \newtheorem*{corollary*}{Corollary}
  \newtheorem*{proposition*}{Proposition}
  \newtheorem*{claim*}{Claim}
  
  \theoremstyle{definition}
  \newtheorem{openproblem}{Open Problem}
  \theoremstyle{remark}
  \newtheorem{remark}[theorem]{Remark}

  \theoremstyle{plain}
  \renewcommand{\qedsymbol}{$\square$}

\theoremstyle{plain}
\newcounter{Game} 
\setcounter{Game}{0}
\newenvironment{game}[1][htb]
    {
    \floatname{algorithm}{Game}% Update algorithm name
    \refstepcounter{Game}%to call the Game pointer. Currently the problem is that caption command by default calls the algorithm pointer. For the moment we need to use Game~~\ref{blah}
   \begin{algorithm}[#1]%
  }{\end{algorithm}}

% ---------------------------------------------------------------------------

%Due to incompatibility between cryptocode and autonum, the following hack is needed. https://tex.stackexchange.com/questions/522666/incompatibility-between-cryptocode-and-autonum:
\expandafter\let\expandafter\savedflalignstar\csname flalign*\endcsname
\expandafter\let\expandafter\savedendflalignstar\csname endflalign*\endcsname
\AtBeginDocument{%
  \expandafter\let\csname flalign*\endcsname\savedflalignstar
  \expandafter\let\csname endflalign*\endcsname\savedendflalignstar
}
\usepackage{tcolorbox}

%Abstract:
%\newcommand{\ab}[1]{#1} \newcommand{\fv}[1]{}

%Full version:
\newcommand{\ab}[1]{} \newcommand{\fv}[1]{#1} %%


\ifnum\masterthesis=1
    \usepackage{setspace}
    \onehalfspacing
    \usepackage{fancyhdr}
    \pagestyle{fancy}
    \fancyhf{}
    \renewcommand{\headrulewidth}{0pt}
    \renewcommand{\headheight}{14pt}
    \chead{\thepage}
    
    \newcommand{\longunderline}{\underline{\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ }\ }
    
    \newenvironment{changemargin}[2]{%
        \begin{list}{}{%
        \setlength{\topsep}{0pt}%
        \setlength{\leftmargin}{#1}%
        \setlength{\rightmargin}{#2}%
        \setlength{\listparindent}{\parindent}%
        \setlength{\itemindent}{\parindent}%
        \setlength{\parsep}{\parskip}%
        }%
    \item[]}{\end{list}}
    
    \newcommand{\logoscale}{0.4}
\fi

\newcommand{\size}[1]{\left|#1\right|}
\newcommand\uprob[2][]{\Pr_{#1}\left[\,#2\,\right]}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% end macros
